Adaptive Second Order Coresets for Data-efficient Machine Learning

Training machine learning models on massive datasets incurs substantial computational costs. To alleviate such costs, there has been a sustained effort to develop data-efficient training methods that can carefully select subsets of the training examples that generalize on par with the full training data. However, existing methods are limited in providing theoretical guarantees for the quality of the models trained on the extracted subsets, and may perform poorly in practice. We propose AdaCore, a method that leverages the geometry of the data to extract subsets of the training examples for efficient machine learning. The key idea behind our method is to dynamically approximate the curvature of the loss function via an exponentially-averaged estimate of the Hessian to select weighted subsets (coresets) that provide a close approximation of the full gradient preconditioned with the Hessian. We prove rigorous guarantees for the convergence of various first and second-order methods applied to the subsets chosen by AdaCore. Our extensive experiments show that AdaCore extracts coresets with higher quality compared to baselines and speeds up training of convex and non-convex machine learning models, such as logistic regression and neural networks, by over 2.9x over the full data and 4.5x over random subsets.

==> extraproof.tex <==
\begin{restatable}{theorem}{pl2restate}
\label{thm:plnew}
    Assume that each loss function $\l_i(w)$ is $\beta$-smooth, $\Lc(w)$ satisfies the $\mu$-PL$^*$ condition in ball $B(w_o,R)$, and $S$ is a weighted subset
    obtained by \alg that estimates the general descent direction by an error of at most $\epsilon$, i.e., $\|\mathbf{H}^{-1}_t \textbf{g}_t-\sum_{j\in S}\gamma_{t,j}\mathbf{H}_{t,j}^{-1} \textbf{g}_{t,j}\|\leq\epsilon$. For R defined as :
    R =  $\frac{2 \beta^3}{ \mu \alpha^3 } \sqrt{\frac{2}{\eta}}  \sqrt{\Lc(w_{0})  - \frac{\beta^2 \epsilon^2}{2\mu} - \frac{\eta \alpha^2}{2} \epsilon + (\frac{\beta}{\mu} + \frac{\alpha^2 \eta}{\beta^2})\epsilon \nabla_{\max} }$. \\
    where $\delta > 0$. Then with probability $1-\delta, SGD with mini-batch size $s \in N$ and step size $\eta^* =\frac{n \mu}{n \beta\left(n^{2} \beta+\mu(s-1)\right)}$ converges to a global solution in the ball $B(w_o,R)$, with an exponential convergence rate:
\begin{align}    
    \Lc(w_{t}) \leq (1-\frac{\eta\mu\alpha^2} {\beta^2})^{t} \Lc(w_0) + \frac{1}{2\mu}(\beta^2\epsilon^2+2\beta\epsilon \nabla_{\max}),
\end{align}
where $\alpha$ is the minimum eigenvalue of all Hessian matrices, and $\nabla_{\max}$ is an upper-bound on the norm of the gradients.
\end{restatable}


\om{working on still}
For the stochastic case need to solve:

    $$
\mathbb{E}\left[\mathcal{L}\left(\mathbf{w}_{t}\right)\right] \leq\left(1-\frac{\mu s \eta^{*}(s)}{n}\right)^{t} \mathcal{L}\left(\mathbf{w}_{0}\right)
$$
Moreover, the expected length of each step is bounded by
$$
\begin{aligned}
\mathbb{E}\left[\left\|\mathbf{w}_{t+1}-\mathbf{w}_{t}\right\|\right] &=\eta^{*} \mathbb{E}\left[\left\|\sum_{j=1}^{s} \nabla \ell_{i_{t}^{(j)}}\left(\mathbf{w}_{t}\right)\right\|\right] \\
& \leq \eta^{*} \sum_{j=1}^{s} \mathbb{E}\left[\left\|\nabla \ell_{i_{t}^{(j)}}\left(\mathbf{w}_{t}\right)\right\|\right] \\
& \leq \eta^{*} \sum_{j=1}^{s} \mathbb{E}\left[\sqrt{2 \lambda \ell_{i_{t}^{(j)}}}\right] \\
& \leq \eta^{*} s \mathbb{E}\left[\sqrt{2 \lambda \mathcal{L}\left(\mathbf{w}_{t}\right)}\right] \\
& \leq \eta^{*} s \sqrt{2 \lambda \mathbb{E}\left[\mathcal{L}\left(\mathbf{w}_{t}\right)\right]} \\
& \leq \eta^{*} s \sqrt{2 \lambda \mathbb{E}\left[(1-\frac{\eta^* s \mu \alpha^2} {n \beta^2})^{t} \Lc(w_0) - \frac{1}{2\mu}(\beta^2\epsilon^2-2\beta\epsilon \nabla_{\max})\right]} \\
& \leq \eta^{*} s \sqrt{2 \lambda (1-\frac{\eta^* s \mu \alpha^2} {n \beta^2})^{t} \Lc(w_0) + \frac{\beta\epsilon \nabla_{\max}}{\mu}} 
\end{aligned}
$$
Note that at the end of the optimization path, we expect that the magnitude of the gradient to go to zero. 
Furthermore, recall.

    From Eq. \eqref{eq:ulb_subset} we have that
    \begin{align*}
        \frac{\|\mathbf{g}_t\|}{\beta}\leq\| (\mathbf{H}_t)^{-1}\mathbf{g}_t\|\leq \| (\mathbf{H}^S_t)^{-1}\mathbf{g}_t^S\pmb\gamma\|+\epsilon \leq \frac{\|\mathbf{g}_t^S\|}{\alpha}+\epsilon
    \end{align*}


By contradiction let $\eps$ not equal to zero. Looking at Eq. \ref{eq:ulb_subset} reproduced above, we have:
    \begin{align*}
        \frac{\|\mathbf{g}_t\|}{\beta}\leq \frac{\|\mathbf{g}_t^S\|}{\alpha}+\epsilon .
    \end{align*}

So at the end of the optimization path, when the magnitude of the gradient goes to zero we have:

    \begin{align*}
        0 \leq \epsilon
    \end{align*}



where we use $\left\{i_{t}^{(1)}, i_{t}^{(2)}, \ldots, i_{t}^{(s)}\right\}$ to denote a random mini-batch of the dataset at step $t$. Then the expectation of the length of the whole optimization path is bounded by
$$
\begin{aligned}
\mathbb{E}\left[\sum_{\tau=0}^{\infty}\left\|\mathbf{w}_{\tau+1}-\mathbf{w}_{\tau}\right\|\right] &=\sum_{\tau=0}^{\infty} \mathbb{E}\left\|\mathbf{w}_{\tau+1}-\mathbf{w}_{\tau}\right\| \\
&=\sum_{\tau=0}^{\infty} \eta^{*} s \sqrt{2 \lambda (1-\frac{\eta^* s \mu \alpha^2} {n \beta^2})^{\tau} \Lc(w_0) - \frac{1}{2\mu}(\beta^2\epsilon^2-2\beta\epsilon \nabla_{\max}(\tau)))} 
\end{aligned}
$$



==> notation_back.tex <==

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\usepackage{xcolor}
\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
% \hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

%--------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{remark}[subsection]{Remark}
\newtheorem{remarks}[subsection]{Remarks}
\newtheorem{example}[subsection]{Example}


%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}

\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\tone}[1]{\|{#1}\|_{\ell_1}}
\newcommand{\eb}{\vct{e}}
\newcommand{\bdd}{\delta}
\newcommand{\be}{\epsilon}
\newcommand{\Scp}{\mathcal{S}_+}
\newcommand{\Scn}{\mathcal{S}_-}
\newcommand{\el}{L}
%\newcommand{\vc}[1]{{\text{vect}(#1)}}
\newcommand{\alpb}{\zeta}
\newcommand{\alpbb}{(\la -\eta\bp^2/2)\bn}
\newcommand{\gam}{{\gamma}}
\newcommand{\KB}{\bar{K}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
%\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\bp}{\beta}
\newcommand{\bn}{\alpha}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\nrest}{\bar{n}}
%\newcommand{\vs}{{\vspace*{-4pt}}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\bt}{\bigotimes}
%\newcommand{\bt}{\times}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}{\text{diag}}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Dc}{{\cal{D}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\btd}{{\bt_{\ell=1}^D d_\ell}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
%\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\bv}{{\boldsymbol{{v}}}}
\newcommand{\bw}{{\boldsymbol{{w}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\stuff}{{\theta}}
\newcommand{\gm}{\gamma_m}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\torder}[1]{\tilde{\cal{O}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{\sigma_{\min}(#1)}}
\newcommand{\smx}[1]{{\sigma_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\tti}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bteta}{\boldsymbol{\theta}}
\newcommand{\bTeta}{\boldsymbol{\Theta}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Mc}{\mathbb{S}^{dr-1}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\all}{{\text{all}}}
%\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
%\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
%\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Fc}{\mathcal{F}}


%%YP's macros
%\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\rbb}{\vct{\bar{r}}}
%\newcommand{\rh}{\vct{\hat{r}}}
%\newcommand{\rt}{\vct{\tilde{r}}}

\newcommand{\qqq}[1]{{\textcolor{black}{{#1}}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}\left(#1\right)}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}{\tilde{\x}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\lipa}{{L}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\avg}[1]{\left< #1 \right>}

\newcommand{\lipp}{\prod_{\ell=1}^D \twonorm{\vct{k}^{(\ell)}}}

\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\rotd}{\text{R1TD}}
\newcommand{\nntd}{\text{DeepTD}}
\newcommand{\x}{\vct{x}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rt}{\tilde{\vct{r}}}
\newcommand{\rbt}{\vct{r}(\vct{\theta})}
\newcommand{\y}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

%\definecolor{emmanuel}{RGB}{255,127,0}
%\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
%\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\renewcommand{\i}{\imath}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}
\newcommand{\bz}{B}
\newcommand{\cp}{R_{p}}
\newcommand{\cs}{\nu}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}


\newcommand{\MS}[1]{\textcolor{blue}{MS: #1}}
\newcommand{\MST}[1]{\textcolor{red}{#1}}
\newcommand{\SO}[1]{\textcolor{darkgreen}{SO: #1}}

%\usepackage{chngcntr}
%\numberwithin{equation}{section} 

\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}
\newenvironment{proof}{\noindent {\bf Proof} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch} }{\endprf\par}


\newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
           \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\red}{\textcolor{red}}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

